AMOEBA: A Coarse Grained Reconfigurable Architecture for Dynamic GPU Scaling

Different GPU applications exhibit varying scalability patterns with network-on-chip (NoC), coalescing, memory and control divergence, and L1 cache behavior. A GPU consists of several StreamingMulti-processors (SMs) that collectively determine how shared resources are partitioned and accessed. Recent years have seen divergent paths in SM scaling towards scale-up (fewer, larger SMs) vs. scale-out (more, smaller SMs). However, neither scaling up nor scaling out can meet the scalability requirement of all applications running on a given GPU system, which inevitably results in performance degradation and resource under-utilization for some applications. In this work, we investigate major design parameters that influence GPU scaling. We then propose AMOEBA, a solution to GPU scaling through reconfigurable SM cores. AMOEBA monitors and predicts application scalability at run-time and adjusts the SM configuration to meet program requirements. AMOEBA also enables dynamic creation of heterogeneous SMs through independent fusing or splitting. AMOEBA is a microarchitecture-based solution and requires no additional programming effort or custom compiler support. Our experimental evaluations with application programs from various benchmark suites indicate that AMOEBA is able to achieve a maximum performance gain of 4.3x, and generates an average performance improvement of 47% when considering all benchmarks tested.

==> description.tex <==
\section{Introduction}

This document provides instructions for submitting papers to the 26th
International Symposium on High Performance Computer Architecture (HPCA), 2020.  In an
effort to respect the efforts of reviewers and in the interest of
fairness to all prospective authors, we request that all submissions
to HPCA 2020 follow the formatting and submission rules detailed
below. Submissions that violate these instructions may not be reviewed,
at the discretion of the program chairs, in order to maintain a review
process that is fair to all potential authors.


An example file (formatted using the HPCA'20 submission format) that
contains the formatting guidelines can be downloaded from the 
\href{https://www.hpca-conf.org/2020/}{HPCA webpage}.  The content of this
document mirrors the submission instructions that appear on that
page.  The link to the HotCRP submission site also appears on the HPCA
webpage.

All questions regarding paper formatting and submission should be directed
to the program co-chairs using the email address \textit{hpca2020pc$@$gmail.com}.

The following formatting guideline is final, but the rest of the policy that is not formatting related has not been finalized. Please refer to the \hbox{\href{https://www.hpca-conf.org/2020/}{HPCA webpage}} for more details.

\subsection{Format Highlights}
Note that there are several notices for paper format:
\begin{itemize}
\item Paper must be submitted in printable PDF format.
\item Text must be in a minimum 10pt ({\bf not} 9pt) font.
\item Papers must be at most 11 pages, not including references. 
\item No page limit for references.
\item The references must include complete author lists (no {\em et al.}).
\end{itemize}


\subsection{Paper Evaluation Objectives}
The committee will make every effort to judge each submitted paper on
its own merits. There will be no target acceptance rate.
We expect to accept a wide range of papers with appropriate expectations
for evaluation --- while papers that build on significant past work
with strong evaluations are valuable, papers that open new areas with
less rigorous evaluation are equally welcome and especially encouraged.
Given the wide range of topics covered by HPCA, every effort will be
made to find expert reviewers.

\subsection{Optional Second PDF for Resubmitted Papers}

For submissions that were previously submitted to other conferences,
we strongly encourage authors to take into account feedback received
from previous reviews.  There is a reasonable probability that an
HPCA-26 submission may be assigned to reviewers that have seen earlier
versions of the same paper.  
\hl{To ease the reviewing burden, and to help authors highlight the
improvements to their paper, authors can optionally submit a second
pdf that highlights the major changes to their work, relative to prior
submissions.}
We anticipate that this process will hold authors and reviewers more
accountable, and perhaps help reduce any pre-conceived bias that a
reviewer may have against the paper.
\begin{itemize}
\item The second pdf will not be made visible to reviewers by default.  If a reviewer believes they have reviewed an earlier version of the paper, they will email the PC Chairs and ask for the second pdf.
\item The second pdf can not introduce new content.  It must be identical to the HPCA-26 submission, but can use color to highlight specific text/captions that are different from prior versions of the paper.  A 100-word appendix may be included to summarize and provide context for the major changes.
\item In latex, text can be highlighted using \hl{ \textbackslash hl\{...\}, as has been done here.}  The submission template already includes the necessary latex packages color and soul.  To remove the highlight, simply set the highlight color to white (example in the latex template).
\item Authors have the flexibility to decide what significant changes they want to highlight to a reviewer.  Obviously, authors will want to draw attention to all prior show-stopping concerns that have been addressed in the new submission.
\item The second pdf upload deadline is also at 5:00pm AoE (Anywhere on Earth) on Tuesday August 6th.  For those planning on working on their paper until the last minute, a one hour grace period is being offered.
\item In case of any questions about this new policy, please feel free to email the PC chairs at: \\ \textit{hpca2020pc$@$gmail.com}.
\end{itemize}


\section{Paper Preparation Instructions}

\subsection{Paper Formatting}

Papers must be submitted in printable PDF format and should contain a
{\bf maximum of 11 pages} of single-spaced two-column text, {\bf not
  including references}.  You may include any number of pages for
references, but see below for more instructions.  If you are using
\LaTeX~\cite{lamport94} to typeset your paper, then we suggest that
you use the template here:
\href{https://www.hpca-conf.org/2020/wp-content/uploads/2019/07/hpca26-latex-template.tar.gz}{\LaTeX~Template}. This
document was prepared with that template.  If you use a different
software package to typeset your paper, then please adhere to the
guidelines given in Table~\ref{table:formatting}.

\begin{scriptsize}
\begin{table}[h!]
  \centering
  \begin{tabular}{|l|l|}
    \hline
    \textbf{Field} & \textbf{Value}\\
    \hline
    \hline
    File format & PDF \\
    \hline
    Page limit & 11 pages, {\bf not including}\\
               & {\bf references}\\
    \hline
    Paper size & US Letter 8.5in $\times$ 11in\\
    \hline
    Top margin & 1in\\
    \hline
    Bottom margin & 1in\\
    \hline
    Left margin & 0.75in\\
    \hline
    Right margin & 0.75in\\
    \hline
    Body & 2-column, single-spaced\\
    \hline
    Space between columns & 0.25in\\
    \hline
    Body font & 10pt\\
    \hline
    Abstract font & 10pt, italicized\\
    \hline
    Section heading font & 12pt, bold\\
    \hline
    Subsection heading font & 10pt, bold\\
    \hline
    Caption font & 9pt (minimum), bold\\
    \hline
    References & 8pt, no page limit, list \\
               & all authors' names\\
    \hline
  \end{tabular}
  \caption{Formatting guidelines for submission. }
  \label{table:formatting}
\end{table}
\end{scriptsize}

\textbf{Please ensure that you include page numbers with your
submission}. This makes it easier for the reviewers to refer to different
parts of your paper when they provide comments.

Please ensure that your submission has a banner at the top of the
title page, similar to
\href{https://www.hpca-conf.org/2020/wp-content/uploads/2019/07/hpca26_sample.pdf}{this one},
which contains the submission number and the notice of
confidentiality.  If using the template, just replace XXX with your
submission number.

\subsection{Content}

\noindent\textbf{\sout{Author List.}} Reviewing will be double blind;
therefore, please do not include any author names on any submitted
documents except in the space provided on the submission form.  You must
also ensure that the metadata included in the PDF does not give away the
authors. If you are improving upon your prior work, refer to your prior
work in the third person and include a full citation for the work in the
bibliography.  For example, if you are building on {\em your own} prior
work in the papers \cite{nicepaper1,nicepaper2,nicepaper3}, you would say
something like: ``While the authors of
\cite{nicepaper1,nicepaper2,nicepaper3} did X, Y, and Z, this paper
additionally does W, and is therefore much better."  Do NOT omit or
anonymize references for blind review.  There is one exception to this: for
your own prior work that appeared in IEEE CAL or workshops without archived
proceedings, as discussed later in this document.

\noindent\textbf{Figures and Tables.} Ensure that the figures and tables
are legible.  Please also ensure that you refer to your figures in the main
text.  Many reviewers print the papers in gray-scale. Therefore, if you use
colors for your figures, ensure that the different colors are highly
distinguishable in gray-scale.

\noindent\textbf{References.}  There is no length limit for references.
{\bf Each reference must explicitly list all authors of the paper.  Papers
not meeting this requirement will be rejected.} Authors of NSF proposals
should be familiar with this requirement. Knowing all authors of related
work will help find the best reviewers. Since there is no length limit
for the number of pages used for references, there is no need to save space
here.

\section{Paper Submission Instructions}

\subsection{Guidelines for Determining Authorship}


IEEE guidelines dictate that authorship should be based on a {\bf
  substantial intellectual contribution}. It is assumed that all
authors have had a significant role in the creation of an article that
bears their names. In particular, the authorship credit must be
reserved only for individuals who have met each of the following
conditions:

\begin{enumerate}

\item Made a significant intellectual contribution to the theoretical
  development, system or experimental design, prototype development,
  and/or the analysis and interpretation of data associated with the
  work contained in the article;

\item Contributed to drafting the article or reviewing and/or revising
  it for intellectual content; and

\item Approved the final version of the article as accepted for
  publication, including references.

\end{enumerate}

A detailed description of the IEEE authorship guidelines and
responsibilities is available
\href{https://www.ieee.org/publications_standards/publications/rights/Section821.html}{here}.
Per these guidelines, it is not acceptable to award {\em honorary }
authorship or {\em gift} authorship. Please keep these guidelines in
mind while determining the author list of your paper.


\subsection{Declaring Authors}

Declare all the authors of the paper upfront. Addition/removal of authors
once the paper is accepted will have to be approved by the program co-chairs,
since it potentially undermines the goal of eliminating conflicts for
reviewer assignment.


\subsection{Areas and Topics}

Authors should indicate these areas on the submission form as
well as specific topics covered by the paper for optimal reviewer match. If
you are unsure whether your paper falls within the scope of HPCA, please
check with the program chair -- HPCA is a broad, multidisciplinary
conference and encourages new topics.

\subsection{Declaring Conflicts of Interest}

Authors must register all their conflicts on the paper submission site.
Conflicts are needed to ensure appropriate assignment of reviewers.
If a paper is found to have an undeclared conflict that causes
a problem OR if a paper is found to declare false conflicts in order to
abuse or ``game'' the review system, the paper may be rejected.

Please declare a conflict of interest (COI) with the following people for any author of your paper:

\begin{enumerate}
\item Your Ph.D. advisor(s), post-doctoral advisor(s), Ph.D. students,
      and post-doctoral advisees, forever.
\item Family relations by blood or marriage, or their equivalent,
      forever (if they might be potential reviewers).
\item People with whom you have collaborated in the last FIVE years, including
\begin{itemize}
\item co-authors of accepted/rejected/pending papers.
\item co-PIs on accepted/rejected/pending grant proposals.
\item funders (decision-makers) of your research grants, and researchers
      whom you fund.
\end{itemize}
\item People (including students) who shared your primary institution(s) in the
last FIVE years.
\item Other relationships, such as close personal friendship, that you think might tend
to affect your judgment or be seen as doing so by a reasonable person familiar
with the relationship.
\end{enumerate}

``Service'' collaborations such as co-authoring a report for a professional
organization, serving on a program committee, or co-presenting
tutorials, do not themselves create a conflict of interest.
Co-authoring a paper that is a compendium of various projects with
no true collaboration among the projects does not constitute a
conflict among the authors of the different projects.

On the other hand, there may be others not covered by the above with
whom you believe a COI exists, for example, an ongoing collaboration
which has not yet resulted in the creation of a paper or proposal.
Please report such COIs; however, you may be asked to justify them.
Please be reasonable. For example, you cannot declare a COI with a
reviewer just because that reviewer works on topics similar to or
related to those in your paper.  The PC Chair may contact co-authors
to explain a COI whose origin is unclear.

We hope to draw most reviewers from the PC and the ERC, but others from the
community may also write reviews.  Please declare all your conflicts (not
just restricted to the PC and ERC).  When in doubt, contact the program
co-chairs.

\subsection{Concurrent Submissions and Workshops}

By submitting a manuscript to HPCA'20, the authors guarantee that the
manuscript has not been previously published or accepted for publication in
a substantially similar form in any conference, journal, or the archived
proceedings of a workshop (e.g., in the ACM digital library) -- see
exceptions below. The authors also guarantee that no paper that contains
significant overlap with the contributions of the submitted paper will be
under review for any other conference or journal or an archived proceedings
of a workshop during the HPCA'20 review period. Violation of any of these
conditions will lead to rejection.

The only exceptions to the above rules are for the authors' own papers
in (1) workshops/posters without archived proceedings such as in the ACM digital
library (or where the authors chose not to have their paper appear in the
archived proceedings), or (2) venues such as IEEE CAL where there is an
explicit policy that such publication does not preclude longer conference
submissions.  In all such cases, the submitted manuscript may ignore the above
work to preserve author anonymity. This information must, however, be provided
on the submission form -- the PC chairs will make this information available to
reviewers if it becomes necessary to ensure a fair review.  As always, if you
are in doubt, it is best to contact the program co-chairs.
        
Authors are not barred from uploading their papers to arxiv and similar sites.
But please note that such efforts may compromise the double-blind review
process, so please exercise care when discussing your submission in public
forums.  On a related note, unrefereed on-line pre-prints are not assumed to
constitute ``prior work'' -- in other words, reviewers cannot penalize an HPCA
submission because it does not cite a pre-print with limited visibility.


Finally, we also note that the IEEE Plagiarism Guidelines \href{http://www.ieee.org/publications\_standards/publications/rights/plagiarism.html}{IEEE Plagiarism Guidelines} covers a range of ethical issues concerning the misrepresentation of other works or
one's own work.

\section{Acknowledgements}
This document is derived from previous conferences, in particular HPCA 2018 and HPCA 2019. 


